NORA: A Harness-Engineered Autonomous Research Agent for End-to-End Spatial Data Science

The automation of scientific research workflows has emerged as a transformative frontier in artificial intelligence, yet existing autonomous research agents remain largely domain-agnostic, lacking the specialized reasoning, method selection, and data acquisition capabilities required for rigorous spatial data science. This paper introduces NORA (Night Owl Research Agent), a harness-engineered, multi-agent autonomous research system purpose-built for GIScience and spatial data science. NORA orchestrates the complete research lifecycle through a skills-first architecture comprising 21 domain-specialized workflow skills, 9 specialist sub-agents, and custom Model Context Protocol (MCP) servers. Central to the system's design are two novel domain-specialized skills: a spatial analysis skill unit that encodes decision frameworks for exploratory spatial data analysis, spatial regression, and diagnostics; and a spatial data download skill that supports reproducible acquisition from authoritative geospatial data sources. We formalize the concept of harness engineering for scientific research agents, demonstrating how lifecycle hooks, safety gates, generator-evaluator separation, human-in-the-loop, and state persistence ensure reliable and reproducible autonomous research. We evaluate NORA through case studies by 6 domain specialists and 3 LLM reviewers across seven dimensions (novelty, quality, rigor, etc). Results demonstrate that domain-specialized harness engineering substantially improves the efficiency and quality of research output compared to general-purpose agent configurations.

==> manuscript_raw.tex <==
Bing Zhou\textsuperscript{a*}, Xiao Huang\textsuperscript{b}, Huan Ning\textsuperscript{b}, Qiusheng Wu\textsuperscript{a}, Diya Li\textsuperscript{c}, Ziyi Zhang\textsuperscript{d}

\emph{\textsuperscript{a} Department of Geography and Sustainability, University of Tennessee, Knoxville, Knoxville, TN}

\emph{\textsuperscript{b} Department of Environmental Science, Emory University, Atlanta, GA}

\emph{\textsuperscript{c} Department of Geography, Texas A\&M University, College Station, TX}

\emph{\textsuperscript{d} TikTok, San Jose, CA}

\textsuperscript{*}Email: bzhou11@utk.edu

\textbf{Abstract}

The automation of scientific research workflows has emerged as a transformative frontier in artificial intelligence, yet existing autonomous research agents remain largely domain-agnostic, lacking the specialized reasoning, method selection, and data acquisition capabilities required for rigorous spatial data science. This paper introduces NORA (Night Owl Research Agent), a harness-engineered, multi-agent autonomous research system purpose-built for GIScience and spatial data science. NORA orchestrates the complete research lifecycle through a skills-first architecture comprising 21 domain-specialized workflow skills, 9 specialist sub-agents, and custom Model Context Protocol (MCP) servers. Central to the system\textquotesingle s design are two novel domain-specialized skills: a spatial analysis skill unit that encodes decision frameworks for exploratory spatial data analysis, spatial regression, and diagnostics; and a spatial data download skill that supports reproducible acquisition from authoritative geospatial data sources. We formalize the concept of harness engineering for scientific research agents, demonstrating how lifecycle hooks, safety gates, generator-evaluator separation, human-in-the-loop, and state persistence ensure reliable and reproducible autonomous research. We evaluate NORA through case studies by 6 domain specialists and 3 LLM reviewers across seven dimensions (novelty, quality, rigor, etc). Results demonstrate that domain-specialized harness engineering substantially improves the efficiency and quality of research output compared to general-purpose agent configurations.

\textbf{Keywords:} research agent, spatial data science, harness engineering, large language models, reproducibility

\section{Introduction}\label{introduction}

The past decade has witnessed an accelerating convergence between artificial intelligence and geographic information science, giving rise to a vibrant research domain variously termed GeoAI (Janowicz et al. 2020), spatial data science (Singleton and Arribas-Bel 2021). This convergence has produced powerful tools for spatial prediction and geospatial knowledge extraction. Yet the process of conducting spatial research itself, which contains formulating hypotheses, acquiring geospatial data, selecting spatially appropriate analytical methods, interpreting results in geographic context, and communicating findings through scholarly manuscripts, remains a predominantly manual, labor-intensive endeavor requiring deep domain expertise at every stage.

Recent advances in large language models (LLMs) and autonomous agents have demonstrated the feasibility of automating substantial portions of scientific research. The AI Scientist (Lu et al. 2026) achieved the milestone of generating a manuscript that passed peer review at a top-tier machine learning workshop, while systems such as Mind2Report (Cheng et al. 2026) have shown that cognitive agentic workflows can synthesize expert-level reports from noisy web sources. In parallel, the Geographic Information Science (GIScience) community has begun exploring LLM-powered spatial agents: LLM-Geo (Li and Ning 2023), LLM-Find (Ning et al. 2025), and GIS Copilot (Akinboyewa et al. 2025) have demonstrated that LLMs can generate and execute geoprocessing workflows through natural language.

However, existing autonomous research agents have largely been conceptualized around the norms of computer science and AI. Although its pipeline offers a useful foundation, it lacks domain-specific elements and reasoning that suit the needs of GIScience and spatial data science (Figure 1). In these fields, research is often constrained not only by model design but also by the discovery, acquisition, and assessment of heterogeneous spatial data, whose availability, scale, temporal resolution, and geographic coverage fundamentally shape the feasibility and validity of analysis. General-purpose AI research agents lack the domain-specific reasoning required for rigorous spatial research: not enforce coordinate reference system (CRS) consistency, test for spatial autocorrelation, select spatially appropriate analytical methods---such as geographically weighted regression (Fotheringham et al. 2002) or multiscale GWR (Fotheringham et al. 2017) instead of ordinary least squares when spatial heterogeneity is present---or ensure that geospatial data provenance meets the reproducibility standards increasingly demanded by GIScience journals (Kedron et al. 2021; Nüst and Pebesma 2021). Moreover, GIScience research is also commonly motivated by societally urgent questions involving hazards, health, and environmental change, for which explanatory insight, actionable decision support, and methodological transparency may be as important as predictive accuracy. Lastly, existing GeoAI agents have primarily focused on task-level spatial operations rather than orchestrating the full arc of a research project from conception to comprehensive reporting.

\includegraphics[width=6.5in,height=3.58125in]{./figures/media/image1.png}

Figure 1. Critical gaps between conventional auto research agents for AI venues and GIScience and spatial data science venues

This paper addresses these gaps by introducing NORA (Night Owl Research Agent), a harness-engineered, multi-agent autonomous research system designed specifically for spatial data science research. NORA is not a general-purpose LLM wrapper or a simple coding assistant. It is a domain-specialized research automation platform whose architecture, skill decomposition, and quality assurance mechanisms are purpose-built for the unique demands of GIScience and spatial data science scholarship. The contributions of this paper are as follows:

(1) We propose NORA with a domain-specialized architecture to orchestrate the complete spatial research lifecycle from literature review through manuscript generation. We introduce two novel skill units---a spatial analysis skill for method selection, diagnostics, and spatial reasoning; and a spatial data download skill supporting reproducible acquisition from authoritative geospatial sources---and argue that such domain decomposition is essential for trustworthy automated spatial research.

(2) We formalize the concept of harness engineering in the context of autonomous research systems for spatial data science, demonstrating how lifecycle hooks, structured state persistence, generator-evaluator separation, human-in-the-loop, and safety gates ensure reliable, reproducible, and auditable research workflows.

(3) We evaluate the performance of NORA by conducting three case studies that target the IJGIS publication with various focuses and difficulties. Details are provided on how NORA orchestrates the entire workflow to demonstrate the contributions of each core architectural unit. The final report generated is evaluated by 6 domain experts and 3 LLM reviewers across seven evaluation dimensions to uncover the current capability boundaries of LLM-based auto research agents.

(4) NORA could be the entryway toward standardized workflow and strengthen reproducibility. Once a tool proves reliable and effective, it begins to shape the broader research workflow itself by encouraging more consistent, transparent, and structured practices. In the context of geospatial research, this could support the development of common benchmarking frameworks that allow methods, datasets, and results to be evaluated under shared standards. Equally important, the tool can automatically document each step of the process, including data acquisition, preprocessing, parameter settings, model training, evaluation, and visualization. The automatic record improves the traceability of results and makes it easier for researchers to replicate, verify, and extend the work.

\section{Related Work}\label{related-work}

\subsection{2.1 LLMs in Scientific Workflows and Autonomous Research Agents}\label{llms-in-scientific-workflows-and-autonomous-research-agents}

The vision of automating scientific discovery has deep roots, from early systems such as DENDRAL for mass spectroscopy interpretation to Waltz and Buchanan's (2009) articulation of closed-loop automated science. Recent advances in large language models (LLMs) and autonomous agents have brought this vision substantially closer to realization. Systems such as \emph{The AI Scientist} (Lu et al. 2026) demonstrated the feasibility of end-to-end research automation, spanning ideation, experimentation, manuscript writing, and even automated peer review, with reported workshop-level acceptance at ICLR 2025. Its automated reviewer suggests that LLM-based quality assessment is approaching human-level reliability. Other efforts further reinforce this trajectory. \emph{Mind2Report} (Cheng et al. 2026) introduced a cognitive deep research workflow with dynamic memory and multi-dimensional reflection for synthesizing commercial reports, outperforming systems such as OpenAI's o3 Deep Research and Google's Gemini Deep Research in quality, reliability, and coverage.

Beyond full end-to-end autonomy, LLMs have also been embedded into specific components of scientific workflows. Tool-augmented language models such as \emph{Toolformer} (Schick et al. 2024) showed that LLMs can learn to call external resources. In the geospatial domain, \emph{Spatial-Agent} (Bao et al. 2026) formalized geo-analytical question answering as a concept transformation problem using GeoFlow Graphs grounded in spatial information theory, demonstrating how LLM-based agents can be adapted to domain-specific analytical settings. At the same time, the notion of the agent harness---the surrounding infrastructure that makes AI agents reliable, controllable, and robust---has emerged as a critical discipline. Anthropic (2025) formalized effective harness patterns for long-running agents, including lifecycle hooks, context compaction, and tool orchestration, highlighting that agent capability depends not only on model intelligence but also on the engineering systems that structure and constrain its operation.

However, autonomous LLM agents can reason, call tools, and generate research artifacts, yet they often lack rigorous provenance, standardized workflows, and discipline-specific guardrails that conventional scientific workflow systems (e.g. KNIME) offer. Additionally, existing autonomous research systems are also largely domain-agnostic. This generality is both a strength and a limitation. While it enables broad applicability, it cannot by itself ensure the level of domain-specific rigor. It is precisely these gaps that motivate the harness engineering approach formalized in this paper.

\subsection{2.2 Autonomous GIS}\label{autonomous-gis}

Recently, a research agenda towards Autonomous GIS has been proposed (Li and Ning 2023), envisioning AI-powered geographic information systems that can independently generate and execute geoprocessing workflows. Following this, several LLM-based spatial agent frameworks have emerged (Li et al. 2025). For example, LLM-Find (Ning et al. 2025) developed an autonomous GIS agent framework for geospatial data retrieval, introducing the "data source handbook" concept, which is structured knowledge package teaching LLMs how to retrieve data from specific sources. GIS Copilot (Akinboyewa et al. 2025) extended this work to integrate LLMs into existing GIS platforms such as QGIS. GeoFlow (Bhattaram et al. 2025) demonstrated agentic workflow automation for geospatial tasks, improving task success by 6.8\% over prior work while reducing token costs. GeoColab (Wu et al. 2025) introduced a multi-agent collaborative framework for geospatial code generation. GeoAnalystBench (Zhang et al. 2025) established a benchmark of 50 Python-based spatial analysis tasks, finding that proprietary models achieve 95\% workflow validity while smaller open-source models achieve only 48.5\%. GeoBenchX (Krechetova and Kochedykov 2025) further benchmarked LLM agents on multistep geospatial tasks, finding that even the best models struggle with complex chains of spatial reasoning.

These GeoAI agents represent important advances in automating spatial operations. However, they focus on task-level execution rather than orchestrating a complete research project. None of them addresses the full lifecycle from research question formulation through peer-reviewed manuscript generation, and none of them incorporates the methodological guardrails that spatial research demands.

\subsection{2.3 Reproducibility and Replicability in GIScience}\label{reproducibility-and-replicability-in-giscience}

Reproducibility and replicability (R\&R) have emerged as central concerns in GIScience. Kedron et al. (2021) examined R\&R opportunities and challenges for geospatial research, while Kedron and Li (2024) further analyzed R\&R from a computational and spatial perspective, identifying factors including training data selection, model design uncertainty, and the inherent spatial heterogeneity of geospatial processes. Nüst and Pebesma (2021) highlighted the gap between reproducibility aspirations and practice in computational geography, emphasizing the need for research compendia that include code, data, and containerized computing environments. Leading journals have adopted data and code sharing policies aligned with FAIR principles (Findable, Accessible, Interoperable, Reusable), yet compliance remains inconsistent (Kedron et al. 2026).

Critically, Kedron et al. (2024) observed that reproducibility solutions disproportionately focus on data analysis, with insufficient attention to data acquisition. This is the phase preceding analysis that profoundly shapes downstream results. This observation directly motivates NORA\textquotesingle s dedicated spatial data download skill unit, which enforces provenance documentation, source authority ranking, and validation checks throughout the data acquisition process.

\section{System Design and Architecture}\label{system-design-and-architecture}

\subsection{3.1 Architecture Overview}\label{architecture-overview}

NORA comprises four architectural layers (User Layer, Skills Layer, Persistence Layer, and Infrastructure Layer) that collectively orchestrate the research (Figure 2). The detailed execution workflow and file generation instructions are illustrated in Appendix A.

\includegraphics[width=6.5in,height=4.03889in]{./figures/media/image2.png}Figure 2: NORA Architectural Design.

\textbf{User Layer} serves as the primary interface between NORA and the user, enabling interaction through structured command execution. These commands encapsulate coordinated sets of skills while providing guidance that improves user experience.

\textbf{Skills Layer} constitutes the core of the framework, orchestrating and executing the functions required for automated research tasks. It comprises 21 Markdown-defined skills that encode procedural knowledge for specific research operations. Rather than functioning as rigid scripts, these skills operate as decision frameworks: they specify relevant considerations, required guardrails, and expected outputs, while allowing the executing agent to determine the most appropriate sequence of actions given the current research context. This layer is further supported by 9 sub-agents dedicated to domain-specific tasks, which are invoked by the skills when specialized reasoning or execution is required.

\textbf{Persistence Layer} stores system prompts, instructional files, state records, and output artifacts. Together, these components guide agent behavior and enable reliable transfer of contextual information across extended, multi-stage research workflows.

\textbf{Infrastructure Layer} provides external tools and computational environment. NORA is implemented within the Claude Code command-line interface (CLI), while allowing expandability. At this layer, MCP servers and external large language models provide specialized tool access and support reviewer--generator separation during the review process. The layer also manages connections to local and remote GPUs and facilitates interoperability with other software.

\subsection{3.2 System Design Principles}\label{system-design-principles}

NORA\textquotesingle s architecture is guided by three design principles: (1) \textbf{Skills-first modularity.} All research workflow logic resides in self-contained Markdown skill files. This design enables maximum flexibility within defined constraints: the agent reads a skill to understand the workflow, then determines the exact action sequence based on the context, which contrasts with template-based approaches that impose fixed execution paths regardless of context. This principle is crucial for enabling the system to leverage the rapidly evolving capabilities of backbone LLMs. (2) \textbf{Domain-specialized reasoning.} Rather than relying on general LLM knowledge of spatial methods, NORA encodes explicit decision frameworks for spatial analysis: when to use geographically weighted regression versus spatial lag models, how to select spatial weights matrices, and when spatial cross-validation is required, etc. The geo-specialist agent embodies deep expertise in spatial statistics, remote sensing, and GeoAI, providing method recommendations grounded in disciplinary conventions. (3) \textbf{Harness Engineering.} NORA\textquotesingle s harness is the scaffolding that governs the agent\textquotesingle s runtime: lifecycle hooks, persistent state, human checkpoints, and declarative configuration. It externalizes cross-cutting concerns, namely, permissioning, logging, checkpointing, and recovery. Harness engineering plays a crucial role because long-horizon autonomous research exceeds any single context window; structured file-based handoffs defeat "context anxiety" (Anthropic, 2025), enforce generator--evaluator separation, and make multi-session runs deterministically resumable. We therefore elevate it to a first-class design principle: skills encode intent and the harness encodes guarantees. More implementation details are provided in Section 4. The screenshot of the demonstration webpage and CLI interface is shown in Figure 3(a) and (b).

\includegraphics[width=3.20181in,height=1.92382in]{./figures/media/image3.png} \includegraphics[width=3.07488in,height=1.91621in]{./figures/media/image4.png}

\begin{quote}
(a) (b)
\end{quote}

Figure 3: Demonstration webpage and CLI interface.

\subsection{3.3 Agent and Skill Design Principles}\label{agent-and-skill-design-principles}

Agent and skills design for autonomous AI research systems should follow a modular, tool-grounded, and provenance-first philosophy. For long-running scientific workflows, agents and skills should be embedded in an external harness rather than relying on the base model to maintain coherence on its own over extended sessions (Anthropic, 2025).

For skill design: instead of single monolithic prompts, the system should decompose research into reusable, domain-aware skills, such as literature review, data acquisition, analysis, visualization, and manuscript drafting, with explicit input-output contracts (Wang et al., 2023). Scientific credibility depends on transparency, each skill execution should also emit structured metadata and workflow provenance so that data sources, parameter settings, intermediate outputs, and decision points can be inspected, audited, and reproduced later (Nüst \& Pebesma, 2021). Detailed principles and items that should be included in skills are demonstrated in Appendix B.

For agent design, agents should interleave reasoning with action and invoke external tools or skills only through well-defined interfaces, since ReAct-style and tool-augmented language models are more effective and interpretable than text-only generation for multi-step problem solving and factual or computational tasks (Schick et al., 2023; Yao et al., 2023). Agents will also be invoked when subtasks, such as peer review, require context isolation to ensure that LLMs do not over-positively react to the content they generate (Anthropic, 2025). Detailed principles and items that should be included in agents are demonstrated in Appendix C.

\subsection{3.4 Research Lifecycle Workflow}\label{research-lifecycle-workflow}

\includegraphics[width=6.49269in,height=3.02377in]{./figures/media/image5.png}Figure 4: NORA's research lifecycle workflow diagram with human checkpoint design.

The NORA workflow is an end-to-end research pipeline that moves from idea formation to final submission through nine major stages and critical human checkpoints (Figure 4). It also allows the user to start and resume at any intermediate stage. Normally, it begins with Launch, where the user provides the research topic, target venue, and major constraints. In Idea Discovery, the system reviews literature, generates candidate ideas, and checks novelty before the user approves the strongest direction. Data Acquisition then gathers the needed datasets, with explicit human authorization required for sensitive access such as API keys, authentication, or very large downloads. The workflow also includes a checkpoint to approve proposed synthetic data before use.

Next, Experiment Execution runs the core analytical or modeling workflow and evaluates outputs. The process then enters Adversarial Review, an iterative quality-control stage where the system stress-tests the work, critiques weaknesses, and revises it for up to four rounds. If the process becomes blocked, a dedicated human intervention step resolves issues such as policy constraints or unreachable reviewers. After this, the Narrative Report synthesizes findings into a coherent interpretation, and the user must approve this report before writing begins.

In Paper Writing, the system converts the approved narrative into manuscript sections with citations and figures. Review and Revise add a second iterative loop, refining the draft through editorial improvement and compliance checks. Finally, Submission packages the manuscript and requires explicit final approval before submission. Beneath all stages sits a harness layer of hooks and persistent memory files, ensuring every stage can resume reliably and maintain context across the entire workflow.

\subsection{3.5 Configuration and Adaptability}\label{configuration-and-adaptability}

NORA\textquotesingle s behavior is governed by a central configuration file. Journal-specific templates encode venue requirements, including word limits, abstract structure, figure specifications, and required methodological elements. This configurability enables NORA to adapt to different research domains within spatial data science and to target different publication venues without architectural changes.

\section{Harness Engineering for Scientific Spatial Research}\label{harness-engineering-for-scientific-spatial-research}

Harness engineering is the discipline of designing the systems, constraints, and feedback loops that surround AI agents to make them reliable in production (Anthropic, 2025). A harness encompasses the complete infrastructure governing agent operation: tool access controls, safety guardrails, feedback mechanisms, observability layers, and state persistence mechanisms. In the context of scientific research agents, we extend this definition to encompass the engineering of constraints, validation gates, and provenance mechanisms that ensure autonomous research outputs meet the methodological standards of the target scientific community.

For spatial data science specifically, harness engineering must address challenges that do not arise in generic agent contexts: ensuring CRS consistency across heterogeneous datasets, checking spatial autocorrelation in model evaluation, enforcing appropriate spatial method selection given data characteristics, and maintaining the provenance chain from raw geospatial data through published claims. NORA implements harness engineering through 5 mechanisms:

\subsection{4.1 Lifecycle hooks}\label{lifecycle-hooks}

This hook-based approach ensures that the state is never lost between sessions, even when sessions terminate unexpectedly, by executing shell scripts. The pre-tool-use hook (pre\_tool\_use.sh) validates every tool invocation before execution, blocking destructive operations (rm -rf, force push), preventing writing files to system directories, and logging all tool calls for audit. The stop hook (stop\_hook.sh) executes on session termination, performing three critical functions: (1) updating persistent memory (MEMORY.md) with current pipeline state, token usage, and section quality scores; (2) writing a structured handoff file (handoff.json) capturing pipeline position, review state, experiment results, and recovery instructions; and (3) triggering notifications.

\subsection{\texorpdfstring{4.2 Generator-evaluator separation }{4.2 Generator-evaluator separation }}\label{generator-evaluator-separation}

NORA enforces that the entity generating content never evaluates its own output. This separation operates at multiple levels. For example, the paper-writer agent drafts sections in one context, while the peer-reviewer agent scores them in a separate context without access to writer reasoning. The mechanism is implemented via MCP (e.g., configurable as GPT via the Codex MCP). Claude Code subagent alternatives are also provided to ensure the main context is quarantined from the review agent when external LLMs are configured erroneously. The review loop implements a scoring mechanism inspired by but extending the automated review approach of The AI Scientist (Lu et al. 2026). Five dimensions are scored on a 0--10 scale: novelty, rigor, literature coverage, clarity, and impact. Acceptance criteria are adjustable, and default to a weighted average score over 7.5, and all five floors are met. The scoring system supports few-shot calibration anchors that link each score level to GIScience-specific examples provided by users. These anchors will ground the scoring in concrete domain expectations.

\subsection{4.3 Structured state persistence}\label{structured-state-persistence}

Rather than relying on LLM context windows and avoiding the risk of information loss during context compression in long-running tasks, NORA persists all critical states to structured files. The handoff.json file captures eight top-level sections: pipeline position (stage, last completed step, next step), review state (per-criterion scores, decision, action items), last experiment results (best model), paper draft state (sections accepted/pending, last score), token budget, and recovery hints (files to read on resume, skill to invoke). On session restart, the orchestrator agent reads handoff.json and deterministically resumes from the exact interruption point, never re-running completed stages or accepted sections.

\subsection{4.4 Human-in-the-loop}\label{human-in-the-loop}

In a domain-specific research pipeline, it is crucial to integrate human checkpoints to ensure the reliability and validity of the generation even when the system is reliable and execute the entire process automatically. The pipeline runs autonomously but pauses at nine deliberate checkpoints (Figure 3): (1) the /launcher intake interview; (2) idea selection after idea-discovery-pipeline; (3) data-download authorization for authentication, API keys, or files above threshold; (4) explicit approval before any fallback to synthetic data; (5) per-round guidance in auto-review-loop; (6) blocked-state resolution on contract violation; (7) narrative-report approval before the paper pipeline; (8) figure-render approval for prompt-pathway diagrams; and (9) final submission confirmation via submit-check. These gates guarantee that autonomous research systems do not blindly self-authorize irreversible decisions. For example, data provenance, fabrication risk, and computing expenditure all require accountable human judgment.

\section{5. Domain-Specialized Skills for Spatial Research}\label{domain-specialized-skills-for-spatial-research}

\subsection{5.1 Rationale for Domain-Specific Skill Decomposition}\label{rationale-for-domain-specific-skill-decomposition}

General-purpose research agents treat all domains equivalently, relying on the LLM\textquotesingle s parametric knowledge to determine appropriate methods. This approach is insufficient for spatial data science for three reasons. First, spatial analysis requires explicit methodological selection. Second, geospatial data acquisition is challenging (Goodchild 2007). Third, spatial research has discipline-specific validity criteria such as Moran\textquotesingle s I of residuals, spatial cross-validation, etc. NORA addresses these requirements through two dedicated skill units that encode domain-specific procedural knowledge: the spatial analysis skill unit and the spatial data download skill unit. NORA also supports easy expansion by adding skills that cover other aspects of spatial data science.

\subsection{5.2 Spatial Analysis Skill Unit}\label{spatial-analysis-skill-unit}

\subsection{The spatial analysis skill unit is a structured decision framework that ensures methods are chosen based on research questions rather than convenience. It includes six connected components. First, it classifies nine analytical objectives (description, explanation, prediction, clustering, accessibility, spatiotemporal change, and causal inference) and links them to appropriate methods. Second, it provides data-readiness guidance for CRS selection, geometry validity, duplicates, dataset integration, and variable preparation, including outlier handling, skewness, multicollinearity, and standardization. Third, it guides the selection of spatial weights and neighbors. Fourth, it offers analytical decision frameworks for regression, clustering, prediction, accessibility, network analysis, and interpolation. For regression, it moves from OLS to residual Moran's I testing and then to spatial lag, spatial error, GWR, or MGWR when appropriate. Fifth, it requires key diagnostics and robustness checks, including residual spatial autocorrelation, heteroscedasticity, MAUP sensitivity, and boundary effects when appropriate. Sixth, it imposes guardrails against common mistakes, such as using latitude/longitude for distance calculations, clustering raw counts, relying on random rather than spatial cross-validation, or overstating causality. This distinguishes NORA from general-purpose agents by embedding explicit, operational spatial reasoning into the workflow.}\label{the-spatial-analysis-skill-unit-is-a-structured-decision-framework-that-ensures-methods-are-chosen-based-on-research-questions-rather-than-convenience.-it-includes-six-connected-components.-first-it-classifies-nine-analytical-objectives-description-explanation-prediction-clustering-accessibility-spatiotemporal-change-and-causal-inference-and-links-them-to-appropriate-methods.-second-it-provides-data-readiness-guidance-for-crs-selection-geometry-validity-duplicates-dataset-integration-and-variable-preparation-including-outlier-handling-skewness-multicollinearity-and-standardization.-third-it-guides-the-selection-of-spatial-weights-and-neighbors.-fourth-it-offers-analytical-decision-frameworks-for-regression-clustering-prediction-accessibility-network-analysis-and-interpolation.-for-regression-it-moves-from-ols-to-residual-morans-i-testing-and-then-to-spatial-lag-spatial-error-gwr-or-mgwr-when-appropriate.-fifth-it-requires-key-diagnostics-and-robustness-checks-including-residual-spatial-autocorrelation-heteroscedasticity-maup-sensitivity-and-boundary-effects-when-appropriate.-sixth-it-imposes-guardrails-against-common-mistakes-such-as-using-latitudelongitude-for-distance-calculations-clustering-raw-counts-relying-on-random-rather-than-spatial-cross-validation-or-overstating-causality.-this-distinguishes-nora-from-general-purpose-agents-by-embedding-explicit-operational-spatial-reasoning-into-the-workflow.}

\subsection{5.3 Spatial Data Download Skill Unit}\label{spatial-data-download-skill-unit}

The spatial data download skill unit addresses an overlooked but crucial part of spatial research: reproducible data acquisition. Responding to Kedron et al.'s argument that geospatial reproducibility efforts focus too heavily on analysis instead of data collection, this skill enforces a six-phase protocol. First, it assesses data needs across ten dimensions, including geography, time, resolution, variables, format, licensing, quality, and size, and maps them to sixteen geospatial data categories. Second, it guides source discovery through a seven-tier hierarchy that prioritizes authoritative and stable providers such as government agencies, international organizations, research repositories, open data projects, APIs, and academic sources. Third, it evaluates candidate sources using nine criteria, including authority, coverage, usability, freshness, stability, and citability. Access controls classify sources as public, API-based, login-restricted, institutional, paid, click-through, or CAPTCHA-protected, forcing human approval when needed. Fourth, it supports multiple download methods, including direct HTTP, APIs, archive extraction, cloud-optimized access, and OpenStreetMap queries, with retry and rate-limiting safeguards. Fifth, it validates downloaded files and checks geographic, temporal, and structural integrity. Sixth, it records every dataset in a DATA\_MANIFEST.md file with detailed provenance fields.

\section{Experiment Design and Evaluation Framework}\label{experiment-design-and-evaluation-framework}

\subsection{6.1 Case Study Design}\label{case-study-design}

We design case studies in which NORA attempts to produce research reports for leading venues in spatial data science, such as the \emph{International Journal of Geographical Information Science (IJGIS).} For each case study, NORA receives a research brief that specifies the topic, target venue, geographic scope, and key datasets. The system then executes the full pipeline autonomously with human checkpoints enabled during execution.

Evaluating an autonomous research agent requires moving beyond the task-level metrics typical of GeoAI benchmarks to assess research-level quality. To this end, we design a multi-faceted evaluation comprising three complementary components: case studies with pipeline analysis, expert and LLM evaluation, and ablation studies.

\subsection{6.2 Expert Evaluation Protocol}\label{expert-evaluation-protocol}

Three domain experts were invited to test NORA and provide qualitative analysis. The experts were selected to cover complementary areas of spatial data science, including spatial statistics, remote sensing, GeoAI, and geographic information systems.

The three experts were asked to monitor the entire research report generation process and record critical behaviors of NORA based on the following guiding questions:

\begin{enumerate}
\def\labelenumi{(\arabic{enumi})}
\item
  Did the agent correctly understand the research objective, scope, target venue, and constraints?
\item
  Did the agent generate ideas that were relevant and non-trivial?
\item
  Did the agent identify the most relevant literature?
\item
  Did the agent identify datasets appropriate for the research question?
\item
  Did the agent correctly clean, transform, and integrate the data?
\item
  Were the chosen methods appropriate for the research question?
\item
  Did the agent execute the workflow correctly and consistently?
\item
  Did the agent demonstrate real domain reasoning rather than generic AI output?
\item
  Did the agent interpret the results correctly and cautiously?
\item
  Were conclusions supported by the evidence?
\item
  Did the agent know when to pause and ask for approval?
\item
  At which stage was the agent strongest and weakest?
\end{enumerate}

To validate the contribution of each core architectural unit, we design ablation studies in which individual components are removed or degraded while the remainder of the system operates normally. The detailed design and study results are recorded in Appendix E.

\subsection{6.3 Evaluation Metrics}\label{evaluation-metrics}

For quantitative assessment, we extend the evaluation metrics from OpenReview, 2024, and focus on the following seven dimensions. Each dimension will be rated from 1 to 10, with 10 being the strongest.

\begin{enumerate}
\def\labelenumi{(\arabic{enumi})}
\item
  \textbf{Idea novelty:} The extent to which the manuscript proposes an original research question, perspective, method, or application that goes beyond well-established or routine work.
\item
  \textbf{Literature coverage:} The degree to which the manuscript identifies, cites, and meaningfully engages with the most relevant prior work in the field.
\item
  \textbf{Significance:} The degree to which the study addresses an important problem and has the potential to make meaningful scientific, practical, or societal impacts.
\item
  \textbf{Code quality:} The extent to which the code is correct, efficient, readable, modular, well-documented, and reproducible for supporting the reported analyses.
\item
  \textbf{Figure quality:} The extent to which figures are accurate, readable, well-designed, and effective in expressing the main findings of the study.
\item
  \textbf{Writing quality:} The degree to which the manuscript is clear, coherent, well-structured, precise, and appropriate in tone for scholarly communication.
\item
  \textbf{Rigor:} The extent to which the study demonstrates methodological soundness, analytical depth, appropriate validation, and careful interpretation of results.
\end{enumerate}

\section{Results and Analysis}\label{results-and-analysis}

\subsection{7.1 Case Study 1: Multi-Vintage Street-View First-Floor Elevation}\label{case-study-1-multi-vintage-street-view-first-floor-elevation}

\textbf{Case and experiment.} This case study asks whether historical Google Street View (GSV) panoramas, treated as a multi-vintage archive rather than a single snapshot, can raise the coverage and decision-utility of community-scale first-floor elevation (FFE) measurement for a barrier-island flood-resilience study in the USA (North Wildwood, NJ). The researcher supplied the direction "use historical street-view images to improve the coverage of first-floor-elevation measurement for North Wildwood, NJ" together with two anchor papers (Ning et al., 2022; Gao et al., 2024) and a 121-image test set with 254 annotated house-front doors for detector benchmarking. The main idea of this method is to measure the elevation of the door bottom as a proxy for the first-floor elevation. NORA executed the full workflow, from literature review to a report with embedded figures, in a single multi-stage session. The study sits in a small but active lineage of street-view first-floor-elevation studies.

The work evaluates a parcel-anchored pipeline over the full residential stock of North Wildwood as represented in OpenStreetMap, namely 1,078 OSM building parcels assigned to 2,199 unique panoramas captured between 2008 and 2022, with Gao et al.\textquotesingle s 2024 YOLOv5 door detector used as a fixed, non-retrained measurement instrument benchmarked against zero-shot Grounding-DINO (Liu et al., 2025). The headline numeric finding, a +15.6 percentage-point coverage gain from latest-only to any-vintage extraction (29.9 \% → 45.5 \%), is conditional on that OSM cohort, and here a notable upstream failure surfaced: NORA did not recognize that OSM building coverage for North Wildwood is materially incomplete relative to a cadastral-parcel inventory, and accordingly missed roughly 80 of the retrievable panoramas. The under-sampling propagates directly into every downstream statistic: the 0-of-29 coverage on FEMA V-zone parcels is most plausibly a lower bound on the true stilted-foundation coverage gap.

\textbf{Human interventions.} Roughly a dozen genuine interventions occurred across the multi-session workflow, of which nine were pipeline-critical. The researcher (1) directed NORA to read the provided reference papers and use the APIs those papers imply for downloading GSV imagery, rather than writing a bespoke client; (2) asked NORA to run an explicit method comparison between a pre-trained YOLO detector and a prompt-based zero-shot model (Grounding-DINO); (3) pointed NORA to the correct code snippets in the relevant GitHub repositories so that the downloader used the supported library calls rather than a reimplementation; (4) provided the no-retraining instruction for the door detector, later reinforced with the clarification that Gao 2024\textquotesingle s checkpoint had already been trained and any retraining would be redundant; (5) supplied information about the pre-installed GPU environment required to run Grounding-DINO; (6) cleared the Windows paging file and enabled GPU use when the first Grounding-DINO inference attempt failed under memory pressure; (7) denied NORA\textquotesingle s request for an OpenTopography academic API key for an external DEM (as used by the reference paper) and redirected NORA to use the EGM96 elevation embedded in each panorama\textquotesingle s metadata as the per-pano ground reference; (8) requested that NORA send detection thumbnails to Codex for adversarial examination of the YOLO and Grounding-DINO outputs; and (9) requested that the necessary figures be inserted into the final report. Each of these interventions kept the pipeline on a scientifically defensible path, and two of them, the redirect away from an external DEM and the library-and-weights pointers, replaced extra work.

\textbf{Case summary.} Extracting first-floor elevation from street-view imagery is non-trivial work that demands intensive skills in programming, data acquisition, and back-and-forth visual and data inspection. From a programming standpoint, NORA significantly reduced the human workload by automating development-environment setup, multi-source data downloading, detector benchmarking, and end-to-end testing; otherwise tedious tasks were automated at low cost. The work still required domain-specific knowledge that NORA did not possess out of the box: it could not independently identify the correct data sources or pre-trained weights without being pointed at them, it did not use perspective-cropped and full-panorama imagery appropriately for the FFE geometry, and it lacked a solid data-inspection instinct for failure modes characteristic of the domain (most visibly, OSM parcel incompleteness relative to a cadastral cohort). Human researchers develop such instincts from accumulated past failures, and NORA currently cannot build equivalent experience on its own because it cannot perform the right quality-control routines without full context on the user\textquotesingle s purpose; it works well when the user supplies timely corrective feedback. Its relatively weak visual capability also limited its performance on image-intensive analyses. In this case, NORA served as a helpful and efficient assistant, yet the user still had to steer the direction at several critical steps.

\subsection{7.2 Case Study 2: Atlanta Crime-Fairness Theorem}\label{case-study-2-atlanta-crime-fairness-theorem}

\textbf{Case and experiment.} This case study investigates whether the choice of spatial algorithm affects not only predictive accuracy but also group-level fairness, using census-tract-level crime prediction in the City of Atlanta. The researcher supplied the direction: \emph{"Atlanta census-tract crime rate prediction with a spatial algorithm using ACS sociodemographic covariates"} and NORA executed the full research workflow from literature review to a submission-ready narrative report in a single session. The resulting study benchmarks seven place-based predictors (OLS, XGBoost, Spatial Lag, Spatial Error, GWR, MGWR, and a Spatial-XGBoost tree baseline that substituted for a GCN after a local torch library failure) against a proven lower bound linking residual Moran\textquotesingle s I, a protected-group clustering coefficient, and a disparate-impact gap. Empirical verification uses 19,494 APD Part-I incidents from 2025 joined at 94.9\% to 169 Atlanta city tracts, paired with ACS 5-year 2018-2022 covariates, plus a 1,000-dataset Monte-Carlo simulation for the theorem and its group-imbalance corollary.

\textbf{Workflow execution by NORA.} NORA launched the /full-pipeline skill, which chained four sub-skills: idea-discovery-pipeline → deploy-experiment → auto-review-loop → generate-report. Idea discovery produced twelve candidates, pruned to six by feasibility-and-novelty filtering, and merged the top three into a unified proposal after a deep novelty-check (score 7.8/10). The refine-research loop reached 8.95/10 over two rounds, and experiment-design produced a plan with five pre-registrations demanded by the internal peer-reviewer sub-agent: a formal theorem statement, block-spatial cross-validation, parameter-count caps, a race-in/race-out covariate ablation, and the demotion of SVC-NN from the contribution list. \emph{deploy-experiment} then ran seventy Atlanta benchmark fits plus the simulation grid, and the adversarial auto-review-loop iterated from 5.0 (ALMOST) in Round 1 to 6.5 (READY) in Round 2, where it corrected a discovered MGWR library-signature bug, added GWR local-coefficient surfaces, documented the analysis CRS, and restructured the paper\textquotesingle s narrative around Corollary 1 and a newly surfaced fold-4 extrapolation finding. Each stage wrote its own structured state to \emph{handoff.json} and \emph{REVIEW\_STATE.json} so the pipeline could survive context compaction, a direct instantiation of NORA\textquotesingle s harness-engineering principles of lifecycle hooks and structured state persistence.

\textbf{Contribution of the spatial analysis and data download skill units.} The spatial analysis skill unit was decisive at several branching points. It enforced an OLS → residual-Moran\textquotesingle s-I → spatial-lag/error → GWR/MGWR progression rather than a monolithic machine-learning sweep, mandated 5-fold block-spatial CV with a two-tract buffer over random splits, defended the use of rook contiguity and the symmetric weight matrix for Moran\textquotesingle s I computation, forced all distance-sensitive operations into EPSG:26967 (NAD83 Georgia West), and required MAUP-consistent residual and fairness diagnostics. The data download skill unit orchestrated three authoritative sources, i.e., TIGER 2020 tract polygons, the Census ACS 5-year API, and the Atlanta Police Department open data portal, and recorded each in data/DATA\_MANIFEST.md with provenance fields including retrieval date, variable list, spatial-join rate, and licensing. When the ArcGIS crime-layer endpoint probes failed, the skill\textquotesingle s validation step flagged the gap explicitly rather than silently proceeding with synthetic stand-in data, enabling the human researcher to supply an authoritative CSV that the protocol then validated, spatial-joined, and merged.

\textbf{Human interventions.} Seven genuine interventions occurred across the full pipeline. The researcher 1) supplied the initial research direction, 2) authorized the creation of a seeded RESEARCH\_PLAN.md, 3) provided the Census API key (stored in a git-ignored .env), 4) supplied the authoritative APD 2025 CSV mid-pipeline, 5) approved Gate 1 after the refined proposal, 6) chose the \emph{reframe} rather than \emph{rescue} option at the Round-1 adversarial-review checkpoint, and 7) requested the final deliverable in Word format. Two of these, i.e., the API key and the real-data CSV, materially improved the reproducibility of the study. Every other decision, including model selection, hyperparameter caps, bug diagnosis and repair, pre-registration tracking, and failure-pivot activation, was made autonomously by NORA under its generator-evaluator-separated architecture.

\textbf{Final report and generated manuscript.} Stage 4 produced NARRATIVE\_REPORT.md together with a matching NARRATIVE\_REPORT.docx (57 KB): twenty-one sections, a ten-row claim-to-evidence matrix citing verbatim numbers, a nine-row figure-and-table plan with five figures already rendered, honest failure-pivot documentation for two pre-registered criteria that did not meet threshold, and twenty verified citation seed keys with no fabricated BibTeX. The narrative is explicitly framed as the contract consumed by NORA\textquotesingle s downstream paper-writing-pipeline, which was left uninvoked in this session so that the case study remains confined to a single end-to-end loop.

\subsection{7.3 Case Study 3: Stochastic Nested Surface Depression Delineation}\label{case-study-3-stochastic-nested-surface-depression-delineation}

\textbf{Case Study and Experiment.} The researcher provided three foundational papers in deterministic surface-depression delineation (Wu et al., 2015; Wu and Lane, 2017; Wu et al., 2018), along with the open-source LiDAR Python package (Wu, 2021), and tasked NORA with generating new research ideas based on this lineage. From ten candidate ideas, NORA selected the question of whether vertical uncertainty in LiDAR-derived digital elevation models (DEMs) can be propagated through nested surface-depression hierarchies in the Prairie Pothole Region (PPR), and whether the resulting probabilistic measures of depression persistence improve predictions of independent surface-water observations. The proposed approach bridges deterministic level-set methods with the per-cell stochastic framework introduced in WhiteboxTools (Lindsay, 2018). NORA implemented the full workflow over the Cottonwood Lake Study Area in North Dakota, using a 3 m USGS 3DEP DEM, Sentinel-1 GRD VV and VH backscatter data (2018--2020), and the JRC Global Surface Water dataset (Pekel et al., 2016). The deterministic baseline identified 5,930 primitive depressions. A Gaussian random field ensemble (N = 25; σ = 0.10 m, ℓ = 60 m) achieved methodological equivalence with WhiteboxTools under matched conditions, yielding a per-depression Spearman correlation of ρ = 0.929. A key finding is a cell-versus-hierarchy decoupling effect. While cell-level persistence remains high (mean = 0.929 across reference depressions), strict parent--child label agreement within the level-set hierarchy shows a median of 0.0 across 577 candidate pairs. This indicates that hierarchical topology is substantially more sensitive to LiDAR vertical uncertainty than the existence of depressions themselves.

\textbf{Workflow execution by NORA.} NORA chained idea-discovery → deploy-experiment → auto-review-loop → generate report. The idea discovery stage produced ten candidate directions and applied an automated novelty assessment, which identified the uncertain merge-tree literature as the primary external risk. An adversarial pre-review then defined the minimum viable contribution and triggered a scope reduction from the 2,770 km² Pipestem subbasin to the Cottonwood Lake HUC12 under a wall-clock constraint. The proposal was subsequently refined with pre-registered success criteria and the Persistence-weighted Inundation Consistency (PwIC) metric formally specified. The experiment deployment stage executed a structured sequence of experiments (R001--R015), including synthetic validation tests, the deterministic baseline, a Gaussian random field (GRF) ensemble, and the WhiteboxTools baseline (Lindsay, 2018). The automated review stage improved to 7.5/10 (Round 2). The pre-registered target (PwIC\_primary ≥ 0.40) was not achieved (Sentinel-1 ρ = 0.164; JRC GSW ρ = 0.250). The contribution was then reframed around three supported findings: methodological equivalence with the Lindsay (2018) baseline, persistence-driven residual signal within size bins, and the decoupling between cell-level persistence and hierarchical structure. Finally, the report generation stage compiled all results.

\textbf{Human interventions.} Five substantive interventions were made by the researcher: (1) providing the foundational papers and LiDAR package, and requesting new research directions without specifying a hypothesis or study area; (2) approving the scope reduction from the Pipestem subbasin to Cottonwood Lake at the pre-review stage; (3) granting access to Google Earth Engine for data retrieval; (4) endorsing the final review decision (Path A), including withdrawal of the strawman claim and deferral of large-scale replication; and (5) requesting the final deliverables in Word format with embedded figures.

\textbf{Final report and generated manuscript.} The final stage produced a comprehensive narrative report, along with a manuscript in both Microsoft Word and PDF formats. Outputs include five core figures and three tables. All results are traceable to structured JSON files at line-level granularity, with both significant and null findings reported. Replication at the full Pipestem extent is explicitly deferred as future work under the validated wall-clock protocol established in the Cottonwood Lake pilot study.

\subsection{7.4 Expert and LLM Evaluation Results}\label{expert-and-llm-evaluation-results}

Six domain experts and three LLM reviewers evaluated the reports generated by NORA across the seven evaluation dimensions illustrated in section 6.3. The results are listed in Table 1.

Table 1. Reports rating from domain experts and LLM reviewers

\begin{longtable}[]{@{}
  >{\centering\arraybackslash}p{(\linewidth - 18\tabcolsep) * \real{0.0961}}
  >{\centering\arraybackslash}p{(\linewidth - 18\tabcolsep) * \real{0.1220}}
  >{\centering\arraybackslash}p{(\linewidth - 18\tabcolsep) * \real{0.0840}}
  >{\centering\arraybackslash}p{(\linewidth - 18\tabcolsep) * \real{0.1444}}
  >{\centering\arraybackslash}p{(\linewidth - 18\tabcolsep) * \real{0.0946}}
  >{\centering\arraybackslash}p{(\linewidth - 18\tabcolsep) * \real{0.1018}}
  >{\centering\arraybackslash}p{(\linewidth - 18\tabcolsep) * \real{0.1104}}
  >{\centering\arraybackslash}p{(\linewidth - 18\tabcolsep) * \real{0.1182}}
  >{\centering\arraybackslash}p{(\linewidth - 18\tabcolsep) * \real{0.0566}}
  >{\centering\arraybackslash}p{(\linewidth - 18\tabcolsep) * \real{0.0720}}@{}}
\toprule\noalign{}
\begin{minipage}[b]{\linewidth}\centering
\textbf{Case No.}
\end{minipage} & \begin{minipage}[b]{\linewidth}\centering
\textbf{Reviewers}
\end{minipage} & \begin{minipage}[b]{\linewidth}\centering
\textbf{Idea Novelty}
\end{minipage} & \begin{minipage}[b]{\linewidth}\centering
\textbf{Literature Coverage}
\end{minipage} & \begin{minipage}[b]{\linewidth}\centering
\textbf{Significance}
\end{minipage} & \begin{minipage}[b]{\linewidth}\centering
\textbf{Code Quality}
\end{minipage} & \begin{minipage}[b]{\linewidth}\centering
\textbf{Figure Quality}
\end{minipage} & \begin{minipage}[b]{\linewidth}\centering
\textbf{Writing Quality}
\end{minipage} & \begin{minipage}[b]{\linewidth}\centering
\textbf{Rigor}
\end{minipage} & \begin{minipage}[b]{\linewidth}\centering
\textbf{Average}
\end{minipage} \\
\midrule\noalign{}
\endhead
\bottomrule\noalign{}
\endlastfoot
\multirow{11}{=}{\centering\arraybackslash Case Study 1} & Reviewer 1 & 5.0 & 6.0 & 5.0 & 6.0 & 7.0 & 4.0 & 4.0 & 5.3 \\
& Reviewer 2 & 6.0 & 6.0 & 5.0 & 6.0 & 7.0 & 4.0 & 7.0 & 5.9 \\
& Reviewer 3 & 7.0 & 9.0 & 5.0 & 6.0 & 7.0 & 6.0 & 5.0 & 6.4 \\
& Reviewer 4 & 8.5 & 9.0 & 8.0 & 9.0 & 8.0 & 8.5 & 8.0 & 8.4 \\
& Reviewer 5 & 5.0 & 4.0 & 4.0 & 6.0 & 5.0 & 7.0 & 3.0 & 4.9 \\
& Reviewer 6 & 6.0 & 4.0 & 7.0 & 7.0 & 4.0 & 2.0 & 1.0 & 4.4 \\
& \textbf{Human Avg} & \textbf{6.3} & \textbf{6.3} & \textbf{5.7} & \textbf{6.7} & \textbf{6.3} & \textbf{5.3} & \textbf{4.7} & \textbf{5.9} \\
& Opus 4.7 & 8.0 & 6.0 & 7.0 & 5.0 & 5.0 & 6.0 & 8.0 & 6.4 \\
& GPT 5.5 & 8.0 & 7.0 & 8.0 & 6.0 & 6.5 & 7.0 & 7.0 & 7.1 \\
& Gemini 3.1 Pro & 8.0 & 8.0 & 8.0 & 7.0 & 8.0 & 9.0 & 9.0 & 8.1 \\
& \textbf{LLM Avg} & \textbf{8.0} & \textbf{7.0} & \textbf{7.7} & \textbf{6.0} & \textbf{6.5} & \textbf{7.3} & \textbf{8.0} & \textbf{7.2} \\
\multirow{11}{=}{\centering\arraybackslash Case Study 2} & Reviewer 1 & 6.0 & 7.0 & 7.0 & 6.0 & 6.0 & 5.0 & 6.0 & 6.1 \\
& Reviewer 2 & 5.0 & 6.0 & 6.0 & 5.0 & 6.0 & 4.0 & 5.0 & 5.3 \\
& Reviewer 3 & 5.0 & 4.0 & 7.0 & 8.0 & 9.0 & 6.0 & 7.0 & 6.6 \\
& Reviewer 4 & 6.0 & 9.0 & 9.0 & 8.5 & 7.0 & 8.5 & 9.0 & 8.1 \\
& Reviewer 5 & 6.0 & 5.0 & 5.0 & 6.0 & 4.0 & 5.0 & 3.0 & 4.9 \\
& Reviewer 6 & 5.0 & 5.0 & 6.0 & 8.0 & 6.0 & 5.0 & 4.0 & 5.6 \\
& \textbf{Human Avg} & \textbf{5.5} & \textbf{6.0} & \textbf{6.7} & \textbf{6.9} & \textbf{6.3} & \textbf{5.6} & \textbf{5.7} & \textbf{6.1} \\
& Opus 4.7 & 6.0 & 8.0 & 7.0 & 7.0 & 8.0 & 8.0 & 8.0 & 7.4 \\
& GPT 5.5 & 8.5 & 8.0 & 8.5 & 7.0 & 8.0 & 9.0 & 7.5 & 8.1 \\
& Gemini 3.1 Pro & 7.0 & 9.0 & 8.0 & 8.0 & 8.0 & 9.0 & 8.0 & 8.1 \\
& \textbf{LLM Avg} & \textbf{7.2} & \textbf{8.3} & \textbf{7.8} & \textbf{7.3} & \textbf{8.0} & \textbf{8.7} & \textbf{7.8} & \textbf{7.9} \\
\multirow{11}{=}{\centering\arraybackslash Case Study 3} & Reviewer 1 & 6.0 & 7.0 & 6.0 & 7.0 & 5.0 & 6.0 & 5.0 & 6.0 \\
& Reviewer 2 & 6.0 & 7.0 & 7.0 & 6.0 & 6.0 & 5.0 & 5.0 & 6.0 \\
& Reviewer 3 & 9.0 & 6.0 & 7.0 & 9.0 & 5.0 & 9.0 & 8.0 & 7.6 \\
& Reviewer 4 & 7.0 & 9.0 & 7.5 & 8.5 & 9.0 & 8.0 & 8.0 & 8.1 \\
& Reviewer 5 & 5.0 & 6.0 & 4.0 & 7.0 & 3.0 & 5.0 & 3.0 & 4.7 \\
& Reviewer 6 & 3.0 & 4.0 & 4.0 & 7.0 & 3.0 & 4.0 & 2.0 & 3.9 \\
& \textbf{Human Avg} & \textbf{6.0} & \textbf{6.5} & \textbf{5.9} & \textbf{7.4} & \textbf{5.2} & \textbf{6.2} & \textbf{5.2} & \textbf{6.0} \\
& Opus 4.7 & 7.0 & 8.0 & 6.0 & 8.0 & 7.0 & 9.0 & 9.0 & 7.7 \\
& GPT 5.5 & 8.5 & 8.5 & 7.5 & 8.0 & 7.5 & 8.0 & 8.0 & 8.0 \\
& Gemini 3.1 Pro & 9.0 & 9.0 & 8.0 & 8.0 & 8.0 & 9.0 & 9.0 & 8.6 \\
& \textbf{LLM Avg} & \textbf{8.2} & \textbf{8.5} & \textbf{7.2} & \textbf{8.0} & \textbf{7.5} & \textbf{8.7} & \textbf{8.7} & \textbf{8.1} \\
\end{longtable}

The evaluation suggests that NORA can produce research manuscripts with moderate-to-strong scholarly quality, but the results also reveal clear areas where human oversight remains necessary. NORA's three generated manuscripts received an overall average score of 6.58/10 across six human reviewers and three LLM evaluators, suggesting a generally promising but uneven level of manuscript quality. Human reviewers were notably more conservative, with an average score of 6.01, compared with 7.73 from the LLM evaluators. This gap is important: while LLMs appear to recognize the structural coherence and apparent completeness of the manuscripts, human reviewers seem more sensitive to disciplinary expectations, especially regarding rigor, interpretation, and scholarly contribution. Across the three case studies, the combined average scores were relatively close, increasing modestly from 6.33 for Case Study 1 to 6.69 for Case Study 2 and 6.73 for Case Study 3, indicating that NORA's performance was reasonably consistent rather than dependent on a single strong case. Among the seven dimensions, code quality received the highest combined score \textbf{(}7.04), followed by literature coverage \textbf{(}6.83), suggesting that NORA is relatively effective at producing technically organized and literature-aware research outputs. However, rigor received the lowest combined score \textbf{(}6.17\textbf{)} and the lowest human-only score \textbf{(}5.17\textbf{)}, highlighting a key limitation: autonomous research agents may generate plausible workflows and polished narratives, but methodological validation and careful interpretation still require expert oversight. The largest human--LLM discrepancies occurred in rigor and writing quality, whereas scores for code quality were nearly identical. Overall, the results position NORA as a useful research acceleration system, but not a substitute for human scholarly judgment.

\section{Discussion}\label{discussion}

\subsection{8.1 Implications for Domain-specific Research Practice}\label{implications-for-domain-specific-research-practice}

NORA shows that domain-specialized autonomous research agents can substantially automate spatial data science workflows while preserving the methodological standards. Its ability to enforce core spatial analysis conventions through explicit, skill-based decision frameworks marks a meaningful advance beyond both general-purpose research agents and task-specific GeoAI tools. The system's harness engineering approach provides a principled foundation for building trustworthy autonomous research systems. By implementing quality assurance mechanisms, NORA makes reliability a property of the surrounding engineering infrastructure rather than relying solely on model capability. This distinction is especially important in spatial data science, because accessible and reliable datasets and the correct selection of spatial methods and evaluation metrics are crucial to ensure scientific rigor. NORA therefore occupies a distinct position within the broader landscape of AI research tools. Compared with The AI Scientist (Lu et al. 2026), NORA exchanges domain generality for spatial specialization. Compared with GIS Copilot (Akinboyewa et al. 2025), NORA moves beyond task-level spatial operations toward full research lifecycle orchestration.

\subsection{8.2 Responsible Automation and Human Oversight}\label{responsible-automation-and-human-oversight}

Based on the case studies, NORA can generate inspiring and novel research ideas and automate experiments. However, responsible automation requires careful identification of where autonomy is appropriate and where human judgment remains necessary. In NORA, several workflow stages are intentionally configured to invite human intervention. These checkpoints performed effectively in the case studies. Technically, these stages could be fully automated by allowing the LLM to select the ``best'' idea, dataset, or method based on predefined criteria. Nevertheless, preserving human checkpoints at these moments helps ensure that the research remains scientifically grounded, ethically aware, and aligned with domain expectations. Human oversight is also necessary when the automated workflow encounters failure or ambiguity. For example, when code execution fails, data acquisition is incomplete, or a required dataset is unavailable, the LLM may attempt to find an alternative data source, modify the analytical strategy, or even reframe the research question. Although such adaptability is useful, these decisions can substantially alter the scope, assumptions, and implications of the study. Human intervention is therefore important to determine whether the modified pathway remains valid.

NORA's generator--evaluator separation and verification gates further support responsible automation by preventing unsupported outputs from moving forward. The LLM-based review mechanism was intentionally strict: when a manuscript or experiment failed to meet the predefined evaluation threshold, the system stopped subsequent tasks rather than forcing completion. Human researchers can still intervene, adjust the threshold, or decide to continue despite a failed review. However, the default behavior prioritizes quality control over productivity. This design reflects a broader principle: autonomous research agents should accelerate scientific work, but they should not bypass accountability, methodological rigor, or human responsibility.

\subsection{8.3 Limitations and Future Directions}\label{limitations-and-future-directions}

Several limitations merit acknowledgment. First, NORA\textquotesingle s quality is bound by the capabilities of its underlying LLMs; as models improve, the system\textquotesingle s output quality will correspondingly advance. Currently, lower performance in non-methodological-focused research, and niche research topics constrain the sophistication of the generated research. Second, the system\textquotesingle s spatial analysis decision frameworks, while comprehensive, inevitably encode a particular methodological perspective; researchers with different analytical traditions may find the default decision paths inappropriately constraining. Third, the adversarial review loop, while more rigorous than self-evaluation, cannot fully substitute for human domain expertise, particularly for assessing conceptual novelty and practical significance. Fourth, the system has been evaluated primarily on spatial regression and remote sensing tasks; its performance on other spatial research paradigms (e.g., human geography, qualitative analysis) remains untested.

Several directions for future work emerge. First, extending NORA\textquotesingle s skill library to additional spatial research paradigms. Second, incorporating multimodal reasoning to enable direct interpretation of maps, satellite imagery, and spatial visualizations. Third, developing collaborative modes where NORA works alongside human researchers in real-time rather than autonomously. Fourth, extending the evaluation framework to include longitudinal studies tracking the impact of NORA-assisted research on research productivity and methodological quality. Fifth, implementing new MCP tools for complicated data harvesting and mechanisms for self-evolving agents and skills. Sixth, enhancing user experience by adapting to multiple CLI tools and building user interfaces.

\subsection{8.4 Pathway toward Reproducibility and Replicability}\label{pathway-toward-reproducibility-and-replicability}

NORA's automation capacity provides a promising pathway toward more reproducible and replicable geospatial research. Once an autonomous research agent becomes reliable enough to support end-to-end scientific workflows, its role extends beyond task assistance; it begins to standardize how research is designed, executed, documented, and evaluated. This is particularly important in spatial data science, where analytical outcomes are often sensitive to data sources, spatial resolution, coordinate reference systems, preprocessing decisions, model parameters, and validation strategies. By encoding these decisions into explicit skills and workflow protocols, NORA can encourage more consistent methodological practices across studies. Moreover, the system can automatically generate detailed records of the research process, including data acquisition procedures, cleaning and transformation steps, spatial analysis choices, model training configurations, evaluation metrics, visualization settings, and intermediate outputs. Such automatic provenance tracking reduces the likelihood that critical methodological details are omitted from manuscripts or supplementary materials. It also makes the research process more transparent, auditable, and easier to rerun by other scholars. In the longer term, systems like NORA could support common benchmarking frameworks for geospatial research, enabling methods, datasets, and findings to be compared under shared standards. In this sense, autonomous research agents may become infrastructure for strengthening scientific accountability rather than merely tools for improving efficiency.

\section{Conclusion}\label{conclusion}

This paper introduced NORA, a harness-engineered autonomous research agent purpose-built for spatial data science. NORA successfully orchestrates the complete research lifecycle, from literature synthesis to adversarial peer review. Crucially, we demonstrated that formalizing harness engineering creates a reliable, reproducible, and auditable foundation for automated scientific workflows.

Our findings underscore that domain decomposition is essential for trustworthy spatial research. Through expert review and ablation analysis, we showed that NORA's domain-specialized architecture is advantageous. The spatial analysis unit effectively prevents common GIScience errors, such as inappropriate method selection and spatial autocorrelation leakage, while the data download unit enforces strict, reproducible data provenance. Furthermore, maintaining a strict separation between generation and evaluation ensures robust result-to-claim verification, actively preventing the propagation of unsupported claims.

Ultimately, NORA represents a critical step toward automating the mechanical aspects of spatial research, including routine analysis, data acquisition, and manuscript formatting. By absorbing these operational tasks, the system frees researchers to concentrate on the creative, conceptual, and ethical dimensions of geographic knowledge production. As the community grapples with the responsible integration of artificial intelligence and the ongoing demand for reproducibility, domain-specialized agents like NORA offer a principled path forward. This approach demonstrates that the future of automated scientific inquiry relies not just on raw model capability, but on the careful engineering of guardrails and quality assurance mechanisms.

\section{Data and Code Availability}\label{data-and-code-availability}

The data and code used in this manuscript, as well as the research agent itself can be accessed through this link: \url{https://github.com/GRIND-Lab-Core/night_owl_research_agent}

\textbf{Declaration of generative AI and AI-assisted technologies in the manuscript preparation process}

During the preparation of this work, the author(s) used ChatGPT and Gemini in order to correct grammatical mistakes and optimize writing. After using this tool/service, the author(s) reviewed and edited the content as needed and take(s) full responsibility for the content of the published article.

\section{References}\label{references}

Akinboyewa, T., Li, Z., Ning, H., \& Lessani, M. N. (2025). GIS Copilot: Towards an autonomous GIS agent for spatial analysis. \emph{International Journal of Digital Earth}, 18(1), 2497489. https://doi.org/10.1080/17538947.2025.2497489

Anthropic. (2025). Effective harnesses for long-running agents. \emph{Anthropic Engineering Blog}, 26 November 2025. https://www.anthropic.com/engineering/effective-harnesses-for-long-running-agents

Bao, R., Yang, C., Yu, D., Tang, Z., Mai, G., \& Zhao, L. (2026). Spatial-Agent: Agentic geo-spatial reasoning with scientific core concepts. arXiv preprint arXiv:2601.16965.

Bhattaram, A., Chung, J., Chung, S., Gupta, R., Ramamoorthy, J., Gullapalli, K., Marculescu, D., \& Stamoulis, D. (2025). GeoFlow: Agentic workflow automation for geospatial tasks. In Proceedings of the 33rd ACM SIGSPATIAL International Conference on Advances in Geographic Information Systems. https://doi.org/10.1145/3748636.3763217

Cheng, M., Wang, D., Liu, Q., Yu, S., Tao, X., Wang, Y., Chu, C., Duan, Y., Long, M., \& Chen, E. (2026). Mind2Report: A cognitive deep research agent for expert-level commercial report synthesis. arXiv preprint arXiv:2601.04879.

Federal Emergency Management Agency. (2011). Coastal Construction Manual: Principles and practices of planning, siting, designing, constructing, and maintaining residential buildings in coastal areas (4th ed., Vol. II, FEMA P-55). U.S. Department of Homeland Security. \url{https://www.fema.gov/sites/default/files/2020-08/fema55_volii_combined_rev.pdf}

Fotheringham, A. S., Brunsdon, C., \& Charlton, M. (2002). Geographically weighted regression: The analysis of spatially varying relationships. Wiley.

Fotheringham, A. S., Yang, W., \& Kang, W. (2017). Multiscale geographically weighted regression (MGWR). Annals of the American Association of Geographers, 107(6), 1247--1265. \url{https://doi.org/10.1080/24694452.2017.1352480}

Gao, G., Ye, X., Li, S., Huang, X., Ning, H., Retchless, D., \& Li, Z. (2024). Exploring flood mitigation governance by estimating first-floor elevation via deep learning and Google Street View in coastal Texas. Environment and Planning B: Urban Analytics and City Science, 51(2), 296--313. https://doi.org/10.1177/23998083231175681

Goodchild, M. F. (2004). The validity and usefulness of laws in geographic information science and geography. Annals of the Association of American Geographers, 94(2), 300--303. https://doi.org/10.1111/j.1467-8306.2004.09402008.x

Goodchild, M. F. (2007). Citizens as sensors: The world of volunteered geography. GeoJournal, 69(4), 211--221. https://doi.org/10.1007/s10708-007-9111-y

Janowicz, K., Gao, S., McKenzie, G., Hu, Y., \& Bhaduri, B. (2020). GeoAI: Spatially explicit artificial intelligence techniques for geographic knowledge discovery and beyond. International Journal of Geographical Information Science, 34(4), 625--636. https://doi.org/10.1080/13658816.2019.1684500

Kedron, P., \& Li, W. (2024). GeoAI reproducibility and replicability: A computational and spatial perspective. Annals of the American Association of Geographers, 114(9), 1925--1945. https://doi.org/10.1080/24694452.2024.2373787

Kedron, P., Bardin, S., Holler, J., \& Turner, B. (2024). Replicable and extensible spatial data acquisition. Cartography and Geographic Information Science, 52(1), 32--48. https://doi.org/10.1080/15230406.2024.2409208

Kedron, P., Li, W., Fotheringham, S., \& Goodchild, M. (2021). Reproducibility and replicability: Opportunities and challenges for geospatial research. International Journal of Geographical Information Science, 35(3), 427--445. \url{https://doi.org/10.1080/13658816.2020.1802032}

Kedron, P., Li, Z., \& Liu, L. (2026). The computational reproducibility of articles published under the Open Data + FAIR policy of IJGIS. International Journal of Geographical Information Science, 0(0), 1--22. \url{https://doi.org/10.1080/13658816.2025.2603586}

Krechetova, V., \& Kochedykov, D. (2025). GeoBenchX: Benchmarking LLMs in agent solving multistep geospatial tasks. In Proceedings of the 1st ACM SIGSPATIAL International Workshop on Generative and Agentic AI for Multi-Modality Space-Time Intelligence (GeoGenAgent \textquotesingle25). https://doi.org/10.1145/3764915.3770721

Li, Z., \& Ning, H. (2023). Autonomous GIS: The next-generation AI-powered GIS. International Journal of Digital Earth, 16(2), 4668--4686. https://doi.org/10.1080/17538947.2023.2278895

Li, Z., Ning, H., Gao, S., Janowicz, K., Li, W., Arundel, S. T., Yang, C., Bhaduri, B., Wang, S., Zhu, A.-X., Gahegan, M., Shekhar, S., Ye, X., McKenzie, G., Cervone, G., \& Hodgson, M. E. (2025a). GIScience in the era of artificial intelligence: A research agenda towards autonomous GIS. Annals of GIS, 31(4), 501--536. \url{https://doi.org/10.1080/19475683.2025.2552161}

Lindsay, J. B. (2018). WhiteboxTools user manual: StochasticDepressionAnalysis. Whitebox Geospatial Inc. \url{https://www.whiteboxgeo.com/}

Liu, S., Zeng, Z., Ren, T., Li, F., Zhang, H., Yang, J., Jiang, Q., Li, C., Yang, J., Su, H., Zhu, J., \& Zhang, L. (2025). Grounding DINO: Marrying DINO with grounded pre-training for open-set object detection. In Computer Vision -- ECCV 2024 (Lecture Notes in Computer Science, pp. 38--55). Springer Nature Switzerland. https://doi.org/10.1007/978-3-031-72970-6\_3

Lovelace, R., Nowosad, J., \& Muenchow, J. (2019). Geocomputation with R. CRC Press. \url{https://doi.org/10.1201/9780203730058}

Lu, C., Lu, C., Lange, R. T., Foerster, J., Clune, J., \& Ha, D. (2024). The AI Scientist: Towards Fully Automated Open-Ended Scientific Discovery (arXiv:2408.06292). arXiv. \url{https://doi.org/10.48550/arXiv.2408.06292}

Lu, C., Lu, C., Lange, R. T., Yamada, Y., Hu, S., Foerster, J., Ha, D., \& Clune, J. (2026). Towards end-to-end automation of AI research. Nature, 651(8107), 914--919. https://doi.org/10.1038/s41586-026-10265-5

Ning, H., Li, Z., Akinboyewa, T., \& Lessani, M. N. (2025). An autonomous GIS agent framework for geospatial data retrieval. International Journal of Digital Earth, 18(1), 2458688. \url{https://doi.org/10.1080/17538947.2025.2458688}

Ning, H., Li, Z., Ye, X., Wang, S., Wang, W., \& Huang, X. (2022). Exploring the vertical dimension of street view image based on deep learning: A case study on lowest floor elevation estimation. International Journal of Geographical Information Science, 36(7), 1317--1342. https://doi.org/10.1080/13658816.2021.1981334

Nüst, D., \& Pebesma, E. (2021). Practical reproducibility in geography and geosciences. Annals of the American Association of Geographers, 111(5), 1300--1310. \url{https://doi.org/10.1080/24694452.2020.1806028}

OpenReview. (2024). Review stage. \href{https://docs.openreview.net/reference/stages/review-stage?utm_source=chatgpt.com}{https://docs.openreview.net/reference/stages/review-stage}

Rey, S. J., \& Anselin, L. (2007). PySAL: A Python library of spatial analytical methods. Review of Regional Studies, 37(1), 5--27.

Schick, T., Dwivedi-Yu, J., Dessì, R., Raileanu, R., Lomeli, M., Hambro, E., Zettlemoyer, L., Cancedda, N., \& Scialom, T. (2024). Toolformer: Language models can teach themselves to use tools. Advances in Neural Information Processing Systems, 36, 68539--68551.

Singleton, A., \& Arribas-Bel, D. (2021). Geographic data science. Geographical Analysis, 53(1), 61--75. https://doi.org/10.1111/gean.12194

Tobler, W. R. (1970). A computer movie simulating urban growth in the Detroit region. Economic Geography, 46(Supplement), 234--240. \url{https://doi.org/10.2307/143141}

Wang, G., Xie, Y., Jiang, Y., Mandlekar, A., Xiao, C., Zhu, Y., Fan, L., \& Anandkumar, A. (2023). Voyager: An Open-Ended Embodied Agent with Large Language Models (arXiv:2305.16291). arXiv. \url{https://doi.org/10.48550/arXiv.2305.16291}

Waltz, D., \& Buchanan, B. G. (2009). Automating science. Science, 324(5923), 43--44. https://doi.org/10.1126/science.1172781

Wu, H., Jiao, H., Hou, S., Liang, J., Shen, Z., Zhao, A., Qing, Y., Jin, F., Guan, X., \& Gui, Z. (2025). GeoColab: An LLM-based multi-agent collaborative framework for geospatial code generation. International Journal of Digital Earth, 18(1), 2569405. \url{https://doi.org/10.1080/17538947.2025.2569405}

Wu, Q. (2021). lidar: A Python package for delineating nested surface depressions from digital elevation data. Journal of Open Source Software, 6(59), 2965. \url{https://doi.org/10.21105/joss.02965}

Wu, Q., \& Lane, C. R. (2017). Delineating wetland catchments and modeling hydrologic connectivity using lidar data and aerial imagery. Hydrology and Earth System Sciences, 21, 3579--3595. \url{https://doi.org/10.5194/hess-21-3579-2017}

Wu, Q., Lane, C. R., Wang, L., Vanderhoof, M. K., Christensen, J. R., \& Liu, H. (2018). Efficient delineation of nested depression hierarchy in digital elevation models for hydrological analysis using level-set method. Journal of the American Water Resources Association, 54(2), 354--371. \url{https://doi.org/10.1111/1752-1688.12689}

Wu, Q., Liu, H., Wang, S., Yu, B., Beck, R., \& Hinkel, K. (2015). A localized contour tree method for deriving geometric and topological properties of complex surface depressions based on high-resolution topographic data. International Journal of Geographical Information Science, 29(12), 2041-2060. \url{https://doi.org/10.1080/13658816.2015.1038719}

Yamada, Y., Lange, R. T., Lu, C., Hu, S., Lu, C., Foerster, J., Clune, J., \& Ha, D. (2025). The AI Scientist-v2: Workshop-Level Automated Scientific Discovery via Agentic Tree Search (arXiv:2504.08066). arXiv. \url{https://doi.org/10.48550/arXiv.2504.08066}

Yao, S., Zhao, J., Yu, D., Du, N., Shafran, I., Narasimhan, K., \& Cao, Y. (2023). ReAct: Synergizing Reasoning and Acting in Language Models (arXiv:2210.03629). arXiv. \url{https://doi.org/10.48550/arXiv.2210.03629}

Zhang, Q., Gao, S., Wei, C., Zhao, Y., Nie, Y., Chen, Z., Chen, S., Su, Y., \& Sun, H. (2025). GeoAnalystBench: A GeoAI benchmark for assessing large language models for spatial analysis workflow and code generation. Transactions in GIS, 29(7), e70135. \url{https://doi.org/10.1111/tgis.70135}

